Contrast with Reconstruct: Contrastive 3D Representation Learning Guided by Generative Pretraining

Mainstream 3D representation learning approaches are built upon contrastive or generative modeling pretext tasks, where great improvements in performance on various downstream tasks have been achieved. However, we find these two paradigms have different characteristics: (i) contrastive models are data-hungry that suffer from a representation over-fitting issue; (ii) generative models have a data filling issue that shows inferior data scaling capacity compared to contrastive models. This motivates us to learn 3D representations by sharing the merits of both paradigms, which is non-trivial due to the pattern difference between the two paradigms. In this paper, we propose Contrast with Reconstruct (ReCon) that unifies these two paradigms. ReCon is trained to learn from both generative modeling teachers and single/cross-modal contrastive teachers through ensemble distillation, where the generative student guides the contrastive student. An encoder-decoder style ReCon-block is proposed that transfers knowledge through cross attention with stop-gradient, which avoids pretraining over-fitting and pattern difference issues. ReCon achieves a new state-of-the-art in 3D representation learning, e.g., 91.26% accuracy on ScanObjectNN. Codes have been released at https://github.com/qizekun/ReCon.

==> tabs/cls/joint_cls_table.tex <==
\begin{table*}[ht!]
\caption{
\textbf{Classification results on the ScanObjectNN and ModelNet40 datasets}. The model parameters number (\#Params), GFLOPS, and overall accuracy (\%) are reported. 
\br Transformer$^{\dagger}$~\citep{AttentionIsAllYouNeed} and \br Point-MAE$^\dagger$~\citep{PointMAE} represent the \textit{from scratch} and \textit{pretrained} (only masked point cloud reconstruction is used) results of our proposed \br\recon-block built backbone architecture, respectively. 
We compare with methods using the \bh hierarchical Transformer architectures (\eg, Point-M2AE~\citep{PointM2AE22}), \bv plain Transformer architectures, and \bs dedicated architectures for 3D point cloud understanding.
}
\label{tab:scanobjectnn}
\begin{center}
\vspace{-14pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[0.95pt]
\multirow{2}{*}[-0.5ex]{Method} & \multirow{2}{*}[-0.5ex]{\#Params (M)} & \multirow{2}{*}[-0.5ex]{GFLOPS} & \multicolumn{3}{c}{ScanObjectNN} & \multicolumn{2}{c}{ModelNet40}\\
\cmidrule(lr){4-6}\cmidrule(lr){7-8} & & & OBJ\_BG & OBJ\_ONLY & PB\_T50\_RS& 1k P & 8k P\\
\midrule[0.6pt]
\multicolumn{8}{c}{\textit{Supervised Learning Only}}\\
\midrule[0.6pt]
\bs PointNet~\citep{PointNet} & 3.5 & 0.5 & 73.3 & 79.2 & 68.0 & 89.2 & 90.8\\
\bs PointNet++~\citep{PointNet++} & 1.5 & 1.7 & 82.3 & 84.3 & 77.9 & 90.7 & 91.9\\
\bs DGCNN~\citep{DGCNN} & 1.8 & 2.4 & 82.8 & 86.2 & 78.1 & 92.9 & -\\
\bs PointCNN~\citep{PointCNN} & 0.6 & - & 86.1 & 85.5 & 78.5 & 92.2 & -\\
\bs DRNet~\citep{DRNet} & - & - & - & - & 80.3 & 93.1 & -\\
\bs SimpleView~\citep{SimpleView} & - & - & - & - & 80.5$\pm$0.3 & 93.9 & -\\
\bs GBNet~\citep{GBNet} & 8.8 & - & - & - & 81.0 & 93.8 & -\\
\bs PRA-Net~\citep{PRANet} & 2.3 & - & - & - & 81.0 & 93.7 & -\\
\bs MVTN~\citep{MVTN} & 11.2 & 43.7 & 92.6 & 92.3 & 82.8 & 93.8 & -\\
\bh PCT~\citep{PCT} & 2.88 & 2.3 & - & - & - & 93.2 & -\\
\bs PointMLP~\citep{PointMLP} & 12.6 & 31.4 & - & - & 85.4$\pm$0.3 & 94.5 & -\\
\bs PointNeXt~\citep{PointNext} & 1.4 & 3.6 & - & - & 87.7$\pm$0.4 & 94.0 & -\\
\bs P2P-RN101~\citep{P2P} & 0.25 & 7.9 & - & - & 87.4 & 93.1 & -\\
\bs P2P-HorNet~\citep{P2P} & 1.2 & 34.6 & - & - & 89.3 & 94.0 & -\\
% Finetuning
\midrule[0.6pt]
\multicolumn{8}{c}{\textit{with Single-Modal Self-Supervised Representation Learning} ({\scshape Full})}\\
\midrule[0.6pt]
\bv Transformer~\citep{AttentionIsAllYouNeed} & 22.1 & 4.8 & 83.04 & 84.06 & 79.11 & 91.4 & 91.8\\
\br Transformer$^\dagger$~\citep{AttentionIsAllYouNeed} & 44.3 & 5.3 & 84.90 & 86.12 & 81.64 & 91.6 & 92.0\\
\bv Point-BERT~\citep{PointBERT} & 22.1 & 4.8 & 87.43 & 88.12 & 83.07 & 93.2 & 93.8\\
\bv MaskPoint~\citep{MaskPoint} & 22.1 & 4.8 & 89.30 & 88.10 & 84.30 & 93.8 & -\\
\bv Point-MAE~\citep{PointMAE} & 22.1 & 4.8 & 90.02 & 88.29 & 85.18 & 93.8 & 94.0\\
\bh Point-M2AE~\citep{PointM2AE22} & 15.3 & 3.6 & 91.22 & 88.81 & 86.43 & 94.0 & -\\
\br Point-MAE$^\dagger$~\citep{PointMAE} & 44.3 & 5.3 & 92.60 & 91.91 & 88.42 & 93.8 & 94.0\\
\rowcolor{linecolor}\br\recon$^\ddagger$~\textbf{w/o vot.} & 44.3 & 5.3 &  &  &  &  & \\
\midrule[0.6pt]
\multicolumn{8}{c}{\textit{with Cross-Modal Self-Supervised Representation Learning} ({\scshape Full})}\\
\midrule[0.6pt]
\bv ACT~\citep{ACT23} & 22.1 & 4.8 & 93.29 & 91.91 & 88.21 & 93.7 & 94.0\\
\rowcolor{linecolor1}\br\recon-Tiny~\textbf{w/o vot.} & 11.4 & 2.4 & \textbf{93.80} & \textbf{92.94} & \textbf{89.10} & 93.3 & 93.6\\
\rowcolor{linecolor2}\br\recon-Small~\textbf{w/o vot.} & 21.0 & 3.2 & \textbf{94.15} & \textbf{93.12} & \textbf{89.52} & 93.5 & 93.8\\
\rowcolor{linecolor}\br\recon\ (scratch teacher)~\textbf{w/o vot.} & 44.3 & 5.3 &  &  &  &  & \\
\rowcolor{linecolor}\br\recon~\textbf{w/o vot.} & 44.3 & 5.3 & \textbf{95.18} & \textbf{93.29} & \textbf{90.63} & \textbf{94.1} & \textbf{94.3}\\
\rowcolor{linecolor}\br\recon~\textbf{w/ vot.} & 44.3 & 5.3 & \textbf{95.35} & \textbf{93.63} & \textbf{91.26} & \textbf{94.5} & \textbf{94.7}\\
% Linear Probing
\midrule[0.6pt]
\multicolumn{8}{c}{\textit{with Self-Supervised Representation Learning} ({\scshape Mlp-Linear})}\\
\midrule[0.6pt]
\br Point-MAE$^\dagger$~\citep{PointMAE} & 44.3 & 5.3 & 82.77$\pm$0.30 & 83.23$\pm$0.16 & 74.13$\pm$0.21 & 90.22$\pm$0.09 & 90.73$\pm$0.09 \\
\bv ACT~\citep{ACT23} & 22.1 & 4.8 & 85.20$\pm$0.83 & 85.84$\pm$0.15 & 76.31$\pm$0.26 & 91.36$\pm$0.17 & 91.75$\pm$0.18 \\
\rowcolor{linecolor}\br\recon & 44.3 & 5.3 & \textbf{89.50}$\pm$0.20 & \textbf{89.72}$\pm$0.17 & \textbf{81.36}$\pm$0.14 & \textbf{92.47}$\pm$0.22 & \textbf{92.68}$\pm$0.07\\
% MLP-3
\midrule[0.6pt]
\multicolumn{8}{c}{\textit{with Self-Supervised Representation Learning} ({\scshape Mlp-3})}\\
\midrule[0.6pt]
\br Point-MAE$^\dagger$~\citep{PointMAE} & 44.3 & 5.3 & 85.78$\pm$0.31 & 85.51$\pm$0.16 & 80.38$\pm$0.21 & 91.25$\pm$0.24 & 91.68$\pm$0.19 \\
\bv ACT~\citep{ACT23} & 22.1 & 4.8 & 87.14$\pm$0.22 & 87.90$\pm$0.40 & 81.52$\pm$0.19 & 92.69$\pm$0.18 & 92.95$\pm$0.10 \\
\rowcolor{linecolor}\br\recon & 44.3 & 5.3 & \textbf{90.62}$\pm$0.22 & \textbf{90.71}$\pm$0.30 & \textbf{83.80}$\pm$0.42& \textbf{93.00}$\pm$0.10 & \textbf{93.39}$\pm$0.05\\
\bottomrule[0.95pt]
\end{tabular}
}
\end{center}
\vspace{-16pt}
\end{table*}

